UADet: A Remarkably Simple Yet Effective Uncertainty-Aware Open-Set Object Detection Framework

We tackle the challenging problem of Open-Set Object Detection (OSOD), which aims to detect both known and unknown objects in unlabelled images. The main difficulty arises from the absence of supervision for these unknown classes, making it challenging to distinguish them from the background. Existing OSOD detectors either fail to properly exploit or inadequately leverage the abundant unlabeled unknown objects in training data, restricting their performance. To address these limitations, we propose UADet, an Uncertainty-Aware Open-Set Object Detector that considers appearance and geometric uncertainty. By integrating these uncertainty measures, UADet effectively reduces the number of unannotated instances incorrectly utilized or omitted by previous methods. Extensive experiments on OSOD benchmarks demonstrate that UADet substantially outperforms previous state-of-the-art (SOTA) methods in detecting both known and unknown objects, achieving a 1.8x improvement in unknown recall while maintaining high performance on known classes. When extended to Open World Object Detection (OWOD), our method shows significant advantages over the current SOTA method, with average improvements of 13.8% and 6.9% in unknown recall on M-OWODB and S-OWODB benchmarks, respectively. Extensive results validate the effectiveness of our uncertainty-aware approach across different open-set scenarios.

==> tables/M-OWODB.tex <==
% \centering
% \small
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}l|cccc|cccc@{}}
%     \midrule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c|}{VOC-COCO-20} & \multicolumn{4}{c}{VOC-COCO-40}  \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%                & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$  & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$  \\ \midrule
%     FR-CNN~\cite{ren2017faster}     & 18.39 & 15118 & 58.45 & 0      & 22.74 & 23391  & 55.26 & 0     \\ 
%     FR-CNN$^*$~\cite{ren2017faster} & 18.83 & 11941 & 57.91 & 0      & 23.24 & 18257  & 54.77 & 0    \\ 
%     PROSER~\cite{zhou2021learning}  & 19.16 & 13035 & 57.66 & 10.92  & 24.15 & 19831  & 54.66 & 7.62  \\
%     ORE~\cite{joseph2021towards}    & 18.18 & 12811 & 58.25 & 2.60   & 22.40 & 19752  & 55.30 & 1.70  \\ 
%     DS~\cite{miller2018dropout}     & 16.98 & 12868 & 58.35 & 5.13   & 20.86 & 19775  & 55.31 & 3.39  \\ 
%     \midrule
%     OpenDet     & \bf{14.95} & \bf{11286} & \bf{58.75} & \bf{14.93} & \bf{18.23} & \bf{16800}  & \bf{55.83} & \bf{10.58} \\ 
%     \midrule
% \end{tabular}%
% }

% \centering
% \small
% \begin{tabular}{@{}l|cccc|cccc@{}}
%     \midrule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c|}{VOC-COCO-20} & \multicolumn{4}{c}{VOC-COCO-40}  \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%                & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$  & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$  \\ \midrule
%     FR-CNN~\cite{ren2017faster}     & 18.39 & 15118 & 58.45 & 0      & 22.74 & 23391  & 55.26 & 0     \\ 
%     FR-CNN$^*$~\cite{ren2017faster} & 18.83 & 11941 & 57.91 & 0      & 23.24 & 18257  & 54.77 & 0    \\ 
%     PROSER~\cite{zhou2021learning}  & 19.16 & 13035 & 57.66 & 10.92  & 24.15 & 19831  & 54.66 & 7.62  \\
%     ORE~\cite{joseph2021towards}    & 18.18 & 12811 & 58.25 & 2.60   & 22.40 & 19752  & 55.30 & 1.70  \\ 
%     DS~\cite{miller2018dropout}     & 16.98 & 12868 & 58.35 & 5.13   & 20.86 & 19775  & 55.31 & 3.39  \\ 
%     \midrule
%     OpenDet     & \bf{14.95} & \bf{11286} & \bf{58.75} & \bf{14.93} & \bf{18.23} & \bf{16800}  & \bf{55.83} & \bf{10.58} \\ 
%     \midrule
% \end{tabular}

% {|l|p{1cm}<{\centering}|*{2}{p{0.75cm}<{\centering}}|*{2}{p{0.75cm}<{\centering}}|}

% \begin{tabular}{@{}l|cccc|cccc@{}}

% \centering
% \small
% \begin{tabular}{l|p{0.2cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.4cm}<{\centering}|p{0.2cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.4cm}<{\centering}}
%     \midrule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c|}{S-OWODB} & \multicolumn{4}{c}{M-OWODB}  \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%                & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & R$_\mathcal{U \uparrow}$  & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & R$_\mathcal{U \uparrow}$  \\ \midrule
%     % FR-CNN~\cite{ren2017faster}     & 18.39 & 15118 & 74.4 & 0      & 22.74 & 23391  & 60.3 & 0     \\ 
%     ORE~\cite{joseph2021towards} & - & - & 61.4 & 1.5    & 6.21 & 10459  & 56.0 & 4.9    \\ 
%     OW-DETR~\cite{gupta2022ow}  & - & - & 71.5 & 5.7  & 5.71 & 10240  & 59.2 & 12.8  \\
%     ALT~\cite{ma2023annealing}    & - & - & - & -   & 6.04 & 8332  & 56.7 & 10.6  \\ 
%     PROB~\cite{zohar2023prob}    & - & - & 73.4 & 17.6   & 4.15 & \bf{5195}  & 59.5 & 19.4  \\ 
%     CAT~\cite{ma2023cat}     & - & - & 74.2 & 24.0  & - & -  & 60.0 & 23.7  \\ 
%     \midrule
%     OpenDet     & \bf{1.54} & \bf{1153} & \bf{75.3} & \bf{30.0} & \bf{3.88} & 5412  & \bf{61.7} & \bf{29.7} \\ 
%     \midrule
% \end{tabular}

% \addtolength{\tabcolsep}{0.5mm}
\begin{center}
% \small
\scriptsize
\begin{tabular}{l|cccc}
\hline
Method & WI$_\downarrow$ & AOSE$_\downarrow$ & mAP$_\mathcal{K \uparrow}$ & R$_\mathcal{U \uparrow}$ \\
\hline
FR-CNN~\cite{ren2017faster} & 22.74 & 23391 & 60.3 & 0 \\
ORE~\cite{joseph2021towards} & 6.21 & 10459 & 56.0 & 4.9 \\
OST~\cite{yang2021objects} & 4.17 & 4889 & 56.2 & - \\
OW-DETR~\cite{gupta2022ow} & 5.71 & 10240 & 59.2 & 12.8 \\
ALT~\cite{ma2023annealing} & 6.04 & 8332 & 56.7 & 10.6 \\
PROB~\cite{zohar2023prob} & 4.15 & \textbf{5195} & 59.5 & 19.4 \\
\hline
CAT~\cite{ma2023cat} & - & - & 60.0 & 23.7 \\
\bf{UPDet} & \textbf{3.88} & 5412 & \textbf{61.7} & \textbf{29.7} \\
$\Delta$ & - & -  & \textcolor{red}{\textbf{+1.7}} & \textcolor{red}{\textbf{+6.0}}\\
\hline
\end{tabular}
\end{center}





==> tables/S-OWODB.tex <==
% \centering
% \small
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}l|cccc|cccc@{}}
%     \midrule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c|}{VOC-COCO-20} & \multicolumn{4}{c}{VOC-COCO-40}  \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%                & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$  & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$  \\ \midrule
%     FR-CNN~\cite{ren2017faster}     & 18.39 & 15118 & 58.45 & 0      & 22.74 & 23391  & 55.26 & 0     \\ 
%     FR-CNN$^*$~\cite{ren2017faster} & 18.83 & 11941 & 57.91 & 0      & 23.24 & 18257  & 54.77 & 0    \\ 
%     PROSER~\cite{zhou2021learning}  & 19.16 & 13035 & 57.66 & 10.92  & 24.15 & 19831  & 54.66 & 7.62  \\
%     ORE~\cite{joseph2021towards}    & 18.18 & 12811 & 58.25 & 2.60   & 22.40 & 19752  & 55.30 & 1.70  \\ 
%     DS~\cite{miller2018dropout}     & 16.98 & 12868 & 58.35 & 5.13   & 20.86 & 19775  & 55.31 & 3.39  \\ 
%     \midrule
%     OpenDet     & \bf{14.95} & \bf{11286} & \bf{58.75} & \bf{14.93} & \bf{18.23} & \bf{16800}  & \bf{55.83} & \bf{10.58} \\ 
%     \midrule
% \end{tabular}%
% }

% \centering
% \small
% \begin{tabular}{@{}l|cccc|cccc@{}}
%     \midrule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c|}{VOC-COCO-20} & \multicolumn{4}{c}{VOC-COCO-40}  \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%                & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$  & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$  \\ \midrule
%     FR-CNN~\cite{ren2017faster}     & 18.39 & 15118 & 58.45 & 0      & 22.74 & 23391  & 55.26 & 0     \\ 
%     FR-CNN$^*$~\cite{ren2017faster} & 18.83 & 11941 & 57.91 & 0      & 23.24 & 18257  & 54.77 & 0    \\ 
%     PROSER~\cite{zhou2021learning}  & 19.16 & 13035 & 57.66 & 10.92  & 24.15 & 19831  & 54.66 & 7.62  \\
%     ORE~\cite{joseph2021towards}    & 18.18 & 12811 & 58.25 & 2.60   & 22.40 & 19752  & 55.30 & 1.70  \\ 
%     DS~\cite{miller2018dropout}     & 16.98 & 12868 & 58.35 & 5.13   & 20.86 & 19775  & 55.31 & 3.39  \\ 
%     \midrule
%     OpenDet     & \bf{14.95} & \bf{11286} & \bf{58.75} & \bf{14.93} & \bf{18.23} & \bf{16800}  & \bf{55.83} & \bf{10.58} \\ 
%     \midrule
% \end{tabular}

% {|l|p{1cm}<{\centering}|*{2}{p{0.75cm}<{\centering}}|*{2}{p{0.75cm}<{\centering}}|}

% \begin{tabular}{@{}l|cccc|cccc@{}}

% \centering
% \small
% \begin{tabular}{l|p{0.2cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.4cm}<{\centering}|p{0.2cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.4cm}<{\centering}}
%     \midrule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c|}{S-OWODB} & \multicolumn{4}{c}{M-OWODB}  \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%                & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & R$_\mathcal{U \uparrow}$  & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & R$_\mathcal{U \uparrow}$  \\ \midrule
%     % FR-CNN~\cite{ren2017faster}     & 18.39 & 15118 & 74.4 & 0      & 22.74 & 23391  & 60.3 & 0     \\ 
%     ORE~\cite{joseph2021towards} & - & - & 61.4 & 1.5    & 6.21 & 10459  & 56.0 & 4.9    \\ 
%     OW-DETR~\cite{gupta2022ow}  & - & - & 71.5 & 5.7  & 5.71 & 10240  & 59.2 & 12.8  \\
%     ALT~\cite{ma2023annealing}    & - & - & - & -   & 6.04 & 8332  & 56.7 & 10.6  \\ 
%     PROB~\cite{zohar2023prob}    & - & - & 73.4 & 17.6   & 4.15 & \bf{5195}  & 59.5 & 19.4  \\ 
%     CAT~\cite{ma2023cat}     & - & - & 74.2 & 24.0  & - & -  & 60.0 & 23.7  \\ 
%     \midrule
%     OpenDet     & \bf{1.54} & \bf{1153} & \bf{75.3} & \bf{30.0} & \bf{3.88} & 5412  & \bf{61.7} & \bf{29.7} \\ 
%     \midrule
% \end{tabular}

% \addtolength{\tabcolsep}{0.5mm}
\begin{center}
% \tiny
\scriptsize
\begin{tabular}{l|cccc}
\hline
Method & WI$_\downarrow$ & AOSE$_\downarrow$ & mAP$_\mathcal{K \uparrow}$ & R$_\mathcal{U \uparrow}$ \\
\hline
FR-CNN~\cite{ren2017faster} & 1.62 & 1448 & 74.4 & 0 \\
ORE~\cite{joseph2021towards} & - & - & 61.4 & 1.5 \\
OW-DETR~\cite{gupta2022ow} & - & - & 71.5 & 5.7 \\
PROB~\cite{zohar2023prob} & - & - & 73.4 & 17.6 \\
\hline
CAT~\cite{ma2023cat} & - & - & 74.2 & 24.0 \\
\bf{UPDet} & \textbf{1.54} & \textbf{1153} & \textbf{75.3} & \textbf{30.0} \\
$\Delta$ & - & - & \textcolor{red}{\textbf{+1.1}} & \textcolor{red}{\textbf{+6.0}}\\
\hline
\end{tabular}
\end{center}





==> tables/ssl_backbone.tex <==
\centering
\small
% \resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{1.3mm}{
\begin{tabular}{c|c|cccc}
\midrule
Backbone & Method      & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & R$_\mathcal{U \uparrow}$  \\ \midrule
\multirow{2}{*}{PixPro~\cite{xie2021propagate}} 
% FR-CNN~\cite{ren2017faster}    & 19.86  & 15509  & 59.56 & 0    \\  
& OpenDet~\cite{han2022expanding}       & 15.88 & \bf{11101} & 58.69 & 36.79 \\
& \bf{Ours}      & \bf{14.70} & 11178 & \bf{59.62} & \bf{61.62}
\\
\hline
\multirow{2}{*}{SloCon~\cite{wen2022self}} 
% FR-CNN~\cite{ren2017faster}    &  18.86 & 16416  & 61.28 & 0    \\  
& OpenDet~\cite{han2022expanding}   & \bf{13.86} & 11049  & 60.49 & 33.23  \\
& \bf{Ours}      & 14.76 & \bf{10327} & \bf{60.81} & \bf{59.30} \\
\midrule
\end{tabular}%
}

==> tables/voc_coco_a_dino.tex <==
% \centering
% \small
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}l|c|ccccc|ccccc|cccccx@{}}
%     \midrule
%     \multirow{2}{*}{Method} & VOC & \multicolumn{5}{c|}{VOC-COCO-20} & \multicolumn{5}{c|}{VOC-COCO-40} & \multicolumn{5}{c}{VOC-COCO-60} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-7}  \cmidrule(lr){8-12} \cmidrule(lr){13-17}
%                 & mAP$_\mathcal{K \uparrow}$ & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$  &  R$_\mathcal{U \uparrow}$  & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$  & 
%                 R$_\mathcal{U \uparrow}$  &
%                 WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$ &
%                 R$_\mathcal{U \uparrow}$  &\\ \midrule
%     FR-CNN~\cite{ren2017faster}    & 80.10 & 18.39 & 15118 & 58.45 & 0 & 0  & 22.74  & 23391  & 55.26  & 0 & 0  & 18.49 & 25472 & 55.83 & 0 & 0      \\ 
%     FR-CNN$^*$~\cite{ren2017faster}& 80.01 & 18.83 & 11941 & 57.91 & 0 & 0   & 23.24 & 18257  & 54.77 & 0 & 0    & 18.72 & 19566 & 55.34 & 0  & 0     \\ 
%     PROSER~\cite{zhou2021learning} & 79.68 & 19.16 & 13035 & 57.66  & 10.92 & 0 & 24.15 & 19831  & 54.66  & 7.62 & 0  & 19.64 & 21322 & 55.20 & 3.25 & 0   \\
%     ORE~\cite{joseph2021towards}   & 79.80 & 18.18 & 12811 & 58.25 & 2.60 & 0  & 22.40 & 19752  & 55.30 & 1.70 & 0 & 18.35 & 21415 & 55.47 & 0.53 & 0   \\ 
%     DS~\cite{miller2018dropout}    & 80.04 & 16.98 & 12868 & 58.35 & 5.13 & 0  & 20.86 & 19775  & 55.31 & 3.39 & 0 & 17.22 & 21921 & 55.77 & 1.25  & 0  \\ 
%     \midrule
%     OpenDet      & 80.02 & \bf{14.95} & \bf{11286} & \bf{58.75} & \bf{14.93} & - & \bf{18.23} & \bf{16800}  & \bf{55.83} & \bf{10.58} & - & \bf{14.24} & \bf{18250} & \bf{56.37} & \bf{4.36} & - \\ 
%     OpenDet(Reproduced) &  &  &  &  &  &  &  &  &  &  &  & & & 0 \\ 
%     Ours &  &  &  &  &  &  &  &  &  &  &  & & & 0\\ 
%     \midrule
% \end{tabular}%
% }

\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|c|ccccc|ccccc|ccccc@{}}
\midrule
\multirow{2}{*}{Method} & VOC & \multicolumn{5}{c|}{VOC-COCO-20} & \multicolumn{5}{c|}{VOC-COCO-40} & \multicolumn{5}{c}{VOC-COCO-60} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-7}  \cmidrule(lr){8-12} \cmidrule(lr){13-17}
                & mAP$_{\mathcal{K} \uparrow}$ & WI$_{\downarrow}$   & AOSE$_{\downarrow}$  & mAP$_{\mathcal{K} \uparrow}$   & AP$_{\mathcal{U} \uparrow}$  &  R$_{\mathcal{U} \uparrow}$  & WI$_{\downarrow}$   & AOSE$_{\downarrow}$  & mAP$_{\mathcal{K} \uparrow}$   & AP$_{\mathcal{U} \uparrow}$  & 
                R$_{\mathcal{U} \uparrow}$  &
                WI$_{\downarrow}$   & AOSE$_{\downarrow}$  & mAP$_{\mathcal{K} \uparrow}$   & AP$_{\mathcal{U} \uparrow}$ &
                R$_{\mathcal{U} \uparrow}$ \\ \midrule
    FR-CNN~\cite{ren2017faster}    & \bf{82.54} & 15.79 & 17272 & \underline{62.37} & 0 & 0  & 19.10  & 26695  & 59.43  & 0 & 0  & 15.09 & 30824 & 60.33 & 0 & 0  \\ 
    PROSER~\cite{zhou2021learning} & 82.30 & 18.44 & 15214 & 61.47  & \bf{20.22} & \underline{43.94} & 22.61 & 23367  & 58.21 & \bf{13.59} & \underline{29.34}  & 17.11 & 25399 & 59.38 & \underline{5.41} & \underline{15.89} \\
    % ORE~\cite{joseph2021towards}   & 79.80 & 18.18 & 12811 & 58.25 & 2.60 & 0  & 22.40 & 19752  & 55.30 & 1.70 & 0 & 18.35 & 21415 & 55.47 & 0.53 & 0   \\ 
    DS~\cite{miller2018dropout}    & \underline{82.43}  & 14.32  & 16329 & 62.35 & 10.23 & 22.21 & 17.52  & 24613 & \underline{59.47} & 6.82 & 14.16 &14.17 & 29119 &  、\underline{60.72} & 2.21 & 5.82    \\
    % ORE~\cite{joseph2021towards}   & 8.39  & 4945  & 77.84 & 1.75   & 15.36 & 10568  & 74.34 & 1.81  & 32.40 & 40865 & 64.59 & 2.14    \\ 
    % PROB~\cite{ma2023annealing} & 81.37 & 16.88 & 18249 & 58.46 & 50.59   & 20.57 & 28365  & 55.89 & 39.17  & 16.27 & 32810 & 56.56 & 25.95 \\
    \midrule
    OpenDet~\cite{han2022expanding}      & 82.12 & \bf{12.03}  & \underline{12486} & 62.09 & 17.05 & 40.76 & \bf{14.47}  & \underline{18219} & 59.32 & 12.02  & 27.26  & \bf{11.52}  & \underline{21969} & 60.18 & 4.81 & 14.90 \\  
    % \midrule
    % OpenDet(Reproduced) & 79.45 & 12.48 & 11613 & 58.29 &  14.47 & 36.01 & 15.18  & 17425 & 55.10 & 10.44 & 24.71 & 12.68 & 20926 & 55.70 & 4.37 & 13.15 \\ 
    \bf{UPDet}  & 82.05 & \underline{12.96} & \bf{12351} & \bf{62.91} & \underline{17.55} & \bf{67.64} & \underline{15.32} & \bf{18178} & \bf{60.16} & \underline{13.42} &\bf{55.66} & \underline{12.03} &  \bf{21531} & \bf{60.98} & \bf{7.40} & \bf{44.21} \\  
    $\Delta$ & \textcolor{red}{\textcolor{blue}{\textbf{-0.07}}} & \textcolor{blue}{\textbf{-0.90}} & \textcolor{red}{\textbf{+135.00}} & \textcolor{red}{\textbf{+0.90}} & \textcolor{red}{\textbf{0.50}} & \textcolor{red}{\textbf{+26.88}} & \textcolor{blue}{\textbf{-0.85}} & \textcolor{red}{\textbf{+41.00}} & \textcolor{red}{\textbf{+0.84}} & \textcolor{red}{\textbf{+1.26}} & \textcolor{red}{\textbf{+28.40}} & \textcolor{blue}{\textbf{-0.51}} & \textcolor{red}{\textbf{+438.00}}  & \textcolor{red}{\textbf{+0.80}} & \textcolor{red}{\textbf{+2.59}} & \textcolor{red}{\textbf{+29.31}}\\ 
    \midrule
\end{tabular}%
}


==> tables/voc_coco_a_old.tex <==
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|ccccc|ccccc|ccccc@{}}
\midrule
\multirow{2}{*}{Method} & VOC & \multicolumn{5}{c|}{VOC-COCO-20} & \multicolumn{5}{c|}{VOC-COCO-40} & \multicolumn{5}{c}{VOC-COCO-60} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-7}  \cmidrule(lr){8-12} \cmidrule(lr){13-17}
                & mAP ($\uparrow$) & \cellcolor[HTML]{FFFFED}{U-Recall ($\uparrow$)} & \cellcolor[HTML]{FFFFED}mAP ($\uparrow$) & WI ($\downarrow$)   & AOSE ($\downarrow$) & U-AP ($\uparrow$)  & \cellcolor[HTML]{FFFFED}{U-Recall ($\uparrow$)} &  \cellcolor[HTML]{FFFFED}mAP ($\uparrow$) & WI ($\downarrow$)   & AOSE ($\downarrow$)  & U-AP ($\uparrow$)   & \cellcolor[HTML]{FFFFED}{U-Recall ($\uparrow$)}  & \cellcolor[HTML]{FFFFED}mAP ($\uparrow$)  & WI ($\downarrow$) & AOSE ($\downarrow$) & U-AP ($\uparrow$) \\ \midrule
    \multicolumn{17}{l}{\textit{Fully-supervised ImageNet-pretrained ResNet50 as Backbone:}} \\ 
    \hline
    FR-CNN$^*$~\cite{ren2017faster}    & 80.06 & \cellcolor[HTML]{FFFFED}0 & \cellcolor[HTML]{FFFFED}58.36 & 19.50 & 16518 & 0 & \cellcolor[HTML]{FFFFED}0  & \cellcolor[HTML]{FFFFED}55.34 & 23.78  & 25339 & 0 & \cellcolor[HTML]{FFFFED}0 & \cellcolor[HTML]{FFFFED}55.94  & 18.91 & 27255 & 0 \\ 
    PROSER$^*$~\cite{zhou2021learning} & 79.42 & \cellcolor[HTML]{FFFFED}37.34 & \cellcolor[HTML]{FFFFED}56.72 & 20.44 & 14266 & \bf{16.99}  & \cellcolor[HTML]{FFFFED}25.10 & \cellcolor[HTML]{FFFFED}53.48  & 25.28 & 21992  & \bf{11.76} & \cellcolor[HTML]{FFFFED}13.02 & \cellcolor[HTML]{FFFFED}54.57  & 20.18 & 23217 & 4.56  \\
    ORE~\cite{joseph2021towards}   & 79.80 & \cellcolor[HTML]{FFFFED}- & \cellcolor[HTML]{FFFFED}58.25 & 18.18 & 12811 & 2.60 & \cellcolor[HTML]{FFFFED}- & \cellcolor[HTML]{FFFFED}55.30 & 22.40 & 19752  & 1.70 & \cellcolor[HTML]{FFFFED}- & \cellcolor[HTML]{FFFFED}55.47 & 18.35 & 21415 & 0.53    \\ 
    DS$^*$~\cite{miller2018dropout}    & 79.70 & \cellcolor[HTML]{FFFFED}19.80 & \cellcolor[HTML]{FFFFED}58.46 & 16.76 & 13062 & 8.75  & \cellcolor[HTML]{FFFFED}12.93 & \cellcolor[HTML]{FFFFED}55.28 & 20.34 & 19891 & 5.94 & \cellcolor[HTML]{FFFFED}5.57  & \cellcolor[HTML]{FFFFED}56.19 & 16.77 & 22406& 2.09 \\ 
    OpenDet$^*$~\cite{han2022expanding} & 80.02 & \cellcolor[HTML]{FFFFED}37.65 & \cellcolor[HTML]{FFFFED}58.64 & \bf{12.50} & 10758 &  14.38  & \cellcolor[HTML]{FFFFED}25.93 & \cellcolor[HTML]{FFFFED}55.60 & \bf{15.38}  & 16061 & 10.49 & \cellcolor[HTML]{FFFFED}14.10 & \cellcolor[HTML]{FFFFED}56.12 & \bf{12.76} & 18548 & 4.37  \\
    OrthogonalDet$^*$~\cite{han2022expanding} & 79.52 & \cellcolor[HTML]{FFFFED}40.65 & \cellcolor[HTML]{FFFFED}58.64 & 14.50 & 10857 & 3.20  & \cellcolor[HTML]{FFFFED}30.93 & \cellcolor[HTML]{FFFFED}55.20 & 18.38  & 16061 & 8.79 & \cellcolor[HTML]{FFFFED}13.10 & \cellcolor[HTML]{FFFFED}56.32 & 15.76 & 18922 & 5.22  \\
    \bf{UADet} & \bf{80.13} & \cellcolor[HTML]{FFFFED}\bf{59.03} & \cellcolor[HTML]{FFFFED}\bf{59.12} & 13.19 & \bf{10186} & 15.09 & \cellcolor[HTML]{FFFFED}\bf{45.28} & \cellcolor[HTML]{FFFFED}\bf{56.00} & 16.17 &  \bf{14956} & 11.51 & \cellcolor[HTML]{FFFFED}\bf{33.49} & \cellcolor[HTML]{FFFFED}\bf{56.73}  & 12.77 & \bf{16550} &  \bf{5.97} \\ 
    \midrule
    \multicolumn{17}{l}{\textit{Self-supervised DINO-pretrained ResNet50 as Backbone:}} \\
    \hline
    PROB$^*$~\cite{han2022expanding} & 79.80 & \cellcolor[HTML]{FFFFED}58.34  & \cellcolor[HTML]{FFFFED}59.91 & 14.33 & 13351 & 3.55 & \cellcolor[HTML]{FFFFED}54.66 & \cellcolor[HTML]{FFFFED}59.26 & 14.32 & 19218 & 13.21 & \cellcolor[HTML]{FFFFED}44.21 & \cellcolor[HTML]{FFFFED}59.72  & 12.03 &  23451 & 2.40 \\  
    \bf{UADet} & 82.05 & \cellcolor[HTML]{FFFFED}\bf{67.64}  & \cellcolor[HTML]{FFFFED}\bf{62.91} & 12.96 & \bf{12351} & \bf{17.55} & \cellcolor[HTML]{FFFFED}\bf{55.66} & \cellcolor[HTML]{FFFFED}\bf{60.16} & 15.32 & \bf{18178} & 13.42 & \cellcolor[HTML]{FFFFED}\bf{44.21} & \cellcolor[HTML]{FFFFED}\bf{60.98}  & 12.03 &  \bf{21531}& \bf{7.40} \\  
    \midrule
\end{tabular}%
}

==> tables/voc_coco_b_dino.tex <==
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|ccccc|ccccc|ccccc@{}}
\midrule
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{VOC-COCO-2500} & \multicolumn{5}{c|}{VOC-COCO-5000} & \multicolumn{5}{c}{VOC-COCO-20000} \\ \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16}
                 & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$  &  R$_\mathcal{U \uparrow}$  & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$  & 
                R$_\mathcal{U \uparrow}$  &
                WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   & AP$_\mathcal{U \uparrow}$ &
                R$_\mathcal{U \uparrow}$ \\ \midrule
FR-CNN~\cite{ren2017faster}    & 7.20  & 6594 &  80.83 & 0 & 0 & 13.22 & 13762  & 76.94 & 0 & 0  &  30.30 & 53708 & 66.68 & 0 & 0     \\ 
% FR-CNN+MSP~\cite{hendrycks2016baseline}    &  & & & & & & & & & & & \\ 
% FR-CNN+MSP~\cite{hendrycks2016baseline}    & 6.90 & 1566 & 77.09 & 29.98 & 12.40 & 3255 & 73.86 & 30.14 & 31.73&12701 & 64.94 & 30.59\\ 
PROSER~\cite{zhou2021learning} & 7.38  & 5694  & 80.10 & \bf{11.76} & 31.89  & 13.92  & 11860 & 76.19 & \underline{14.57} & \underline{32.29} & 30.64  & 46370 & 65.36  & \underline{18.46} & \underline{32.52}  \\
DS~\cite{miller2018dropout}    & 6.17  & 5958  & \underline{81.20} & 5.04 & 17.32 &  11.94 & 12316  & 77.04 & 7.48 & 17.55  & 27.63 & 48126 & 66.45 & 10.82 & 17.41    \\ 
% ORE~\cite{joseph2021towards}   & 8.39  & 4945  & 77.84 & 1.75   & 15.36 & 10568  & 74.34 & 1.81  & 32.40 & 40865 & 64.59 & 2.14    \\ 
\midrule
OpenDet~\cite{han2022expanding}  &  \underline{5.44} & \underline{4285} & 81.17 & 9.47 & \underline{32.09}  & \underline{9.87}   & \underline{8811}  & \underline{78.13} & 12.90 & 31.87 & \underline{24.88} & \underline{34424} & \underline{68.84} & 17.95 & 32.06 \\ 
\bf{UPDet}  & \bf{5.01} & \bf{4230} & \bf{81.60} & \underline{11.38} & \bf{63.07} & \bf{9.19} & \bf{8766}  & \bf{78.36} & \bf{15.00} & \bf{61.57} & \bf{22.72} & \bf{34234} & \bf{68.90} & \bf{20.26} & \bf{62.73} \\ 
$\Delta$ & \textcolor{red}{\textbf{+0.43}} & \textcolor{red}{\textbf{+55}} & \textcolor{red}{\textbf{+0.43}} & \textcolor{red}{\textbf{+1.91}} & \textcolor{red}{\textbf{+30.98}} & \textcolor{red}{\textbf{+0.68}}  & \textcolor{red}{\textbf{+45}} & \textcolor{red}{\textbf{+0.23}} & \textcolor{red}{\textbf{+2.10}} & \textcolor{red}{\textbf{+29.70}} & \textcolor{red}{\textbf{+2.16}}  & \textcolor{red}{\textbf{+190}} & \textcolor{red}{\textbf{+0.06}} & 
\textcolor{red}{\textbf{+2.31}} & \textcolor{red}{\textbf{+30.67}}\\ 
    \midrule
\end{tabular}%
}

% \centering
% \small
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}l|ccccc|ccccc|ccccc@{}}
% \midrule
% \multirow{2}{*}{Method} & \multicolumn{5}{c|}{VOC-COCO-2500} & \multicolumn{5}{c|}{VOC-COCO-5000} & \multicolumn{5}{c}{VOC-COCO-20000} \\ \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16}
%                & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$ & AP$_\mathcal{U \uparrow}$  & R$_\mathcal{U \uparrow}$  & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$ & AP$_\mathcal{U \uparrow}$   & R$_\mathcal{U \uparrow}$  & WI$_\downarrow$   & AOSE$_\downarrow$  & mAP$_\mathcal{K \uparrow}$   &  AP$_\mathcal{U \uparrow}$ & R$_\mathcal{U \uparrow}$  \\ \midrule
% FR-CNN~\cite{ren2017faster}    & 7.20  & 6594 &  80.83 & 0    & -  & 13.22 & 13762  & 76.94 & 0  & -    &  30.30 & 53708 & 66.68 & 0 & -       \\ 
% % FR-CNN+MSP~\cite{hendrycks2016baseline}    &  & & & & & & & & & & & \\ 
% % FR-CNN+MSP~\cite{hendrycks2016baseline}    & 6.90 & 1566 & 77.09 & 29.98 & 12.40 & 3255 & 73.86 & 30.14 & 31.73&12701 & 64.94 & 30.59\\ 
% PROSER~\cite{zhou2021learning} & 7.38  & 5694  & 80.10 & 31.89  & 13.92  & 11860 & 76.19 & 32.29 & 30.64  & 46370 & 65.36  & 32.52  \\
% DS~\cite{miller2018dropout}    & 6.17  & 5958  & 81.20 & 17.32   &  11.94 & 12316  & 77.04 & 17.55  & 27.63 & 48126 & 66.45 &  17.41    \\ 
% % ORE~\cite{joseph2021towards}   & 8.39  & 4945  & 77.84 & 1.75   & 15.36 & 10568  & 74.34 & 1.81  & 32.40 & 40865 & 64.59 & 2.14    \\ 
% OpenDet~\cite{han2022expanding}  &  5.17 & 4360 & 81.50 & 31.13  & 10.19   & 9012  & 78.20 & 30.62 &  24.13 & 35069 & \bf{68.63} & 31.11 \\ 
% \midrule

% Ours  & \bf{5.02} & \bf{4230} & \bf{81.60} & \bf{63.53} & \bf{9.21} & \bf{8808}  & \bf{78.22} & \bf{61.87} & \bf{22.86} & \bf{34447} & 68.62 & \bf{62.73} \\ 
% \midrule
% \end{tabular}%
% }

==> tables/voc_coco_b_old.tex <==
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccccc|ccccc|ccccc}
\midrule
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{VOC-COCO-2500} & \multicolumn{5}{c|}{VOC-COCO-5000} & \multicolumn{5}{c}{VOC-COCO-20000} \\ \cmidrule(lr){2-6}  \cmidrule(lr){7-11} \cmidrule(lr){12-16}
                 & \cellcolor[HTML]{FFFFED}U-Recall ($\uparrow$) & \cellcolor[HTML]{FFFFED}mAP ($\uparrow$)  & WI ($\downarrow$)   & AOSE ($\downarrow$) & U-AP ($\uparrow$)  &  \cellcolor[HTML]{FFFFED}U-Recall ($\uparrow$) & \cellcolor[HTML]{FFFFED}mAP ($\uparrow$) & WI ($\downarrow$)   & AOSE ($\downarrow$) & U-AP ($\uparrow$) & \cellcolor[HTML]{FFFFED}U-Recall ($\uparrow$)  & \cellcolor[HTML]{FFFFED}mAP ($\uparrow$) &
                WI ($\downarrow$)   & AOSE ($\downarrow$)  & U-AP ($\uparrow$) \\ \midrule
\multicolumn{7}{l}{\textit{Fully-supervised ImageNet-pretrained ResNet50 as Backbone:}} \\ 
\hline
FR-CNN$^*$~\cite{ren2017faster}    & \cellcolor[HTML]{FFFFED}0  & \cellcolor[HTML]{FFFFED}77.83 & 9.12  & 6424 & 0 & \cellcolor[HTML]{FFFFED}0 & \cellcolor[HTML]{FFFFED}74.61 & 16.63 & 13499  & 0 & \cellcolor[HTML]{FFFFED}0 & \cellcolor[HTML]{FFFFED}64.50 & 33.90 & 52624 & 0    \\ 
PROSER$^*$~\cite{zhou2021learning} & \cellcolor[HTML]{FFFFED}28.57 & \cellcolor[HTML]{FFFFED}76.76  & 9.68 & 5554 & \bf{10.98} & \cellcolor[HTML]{FFFFED}13.27 & \cellcolor[HTML]{FFFFED}72.75  & 28.38 & 11669  & 17.48 & \cellcolor[HTML]{FFFFED} 28.55  & \cellcolor[HTML]{FFFFED}61.52 &35.64 & 45507 & 16.74   \\
ORE~\cite{joseph2021towards}   & \cellcolor[HTML]{FFFFED}- & \cellcolor[HTML]{FFFFED}77.84 & 8.39  & 4945  & 1.75 & \cellcolor[HTML]{FFFFED}-  & \cellcolor[HTML]{FFFFED}74.34 & 15.36 & 10568  & 1.81 & \cellcolor[HTML]{FFFFED}- & \cellcolor[HTML]{FFFFED}64.59 & 32.40 & 40865 & 2.14   \\ 
DS$^*$~\cite{miller2018dropout}  & \cellcolor[HTML]{FFFFED}16.47 & \cellcolor[HTML]{FFFFED}77.69  & 8.28  & 4917 & 4.76 & \cellcolor[HTML]{FFFFED}16.49 & \cellcolor[HTML]{FFFFED}74.29 & 15.16 & 10226 & 6.73 & \cellcolor[HTML]{FFFFED}16.73 & \cellcolor[HTML]{FFFFED}64.02 & 31.50 & 39870 & 9.90   \\ 
\midrule
\multicolumn{7}{l}{\textit{Self-supervised DINO-pretrained ResNet50 as Backbone:}} \\
\hline
OpenDet$^*$~\cite{han2022expanding} & \cellcolor[HTML]{FFFFED}30.87 & \cellcolor[HTML]{FFFFED}78.65 & 6.14 & 3781 & 8.69 &  \cellcolor[HTML]{FFFFED}30.46 & \cellcolor[HTML]{FFFFED}75.38 & 11.07 & 7819  & 12.21 & \cellcolor[HTML]{FFFFED}30.90 & \cellcolor[HTML]{FFFFED}\bf{65.54} & \bf{24.43} & 30500 & 17.02 \\
\bf{UADet}  & \cellcolor[HTML]{FFFFED}\bf{51.92} & \cellcolor[HTML]{FFFFED}\bf{78.66} & \bf{5.93} & \bf{3476} & 10.02 &  \cellcolor[HTML]{FFFFED}\bf{51.12} &  \cellcolor[HTML]{FFFFED}\bf{75.40}  & \bf{10.82}  & \bf{7308} & \bf{13.18} & \cellcolor[HTML]{FFFFED}\bf{51.58} &  \cellcolor[HTML]{FFFFED}65.43 & 25.10 & \bf{28536} & \bf{17.87} \\
\midrule
\end{tabular}%
}
